Deciding Indistinguishability

Computational indistinguishability is a key property in cryptography and verification of security protocols. Current tools for proving it rely on cryptographic game transformations. We follow Bana and Comon's approach, axiomatizing what an adversary cannot distinguish. We prove the decidability of a set of first-order axioms that are both computationally sound and expressive enough. This can be viewed as the decidability of a family of cryptographic game transformations. Our proof relies on term rewriting and automated deduction techniques.

==> cca-ext.tex <==
\subsubsection{Decryption Oracle Calls}

Any decryption oracle call term is of the form:
\[
  \ite{\big(\bigvee_{i \le n}\eq{s}{\alpha_{i}}\big)}
  {\zero(s)}
  {\dec(s,\sk)}
\]
\begin{wrapfigure}{r}{7cm}
  \vspace{-2em}
  \begin{center}
    \begin{tikzpicture}
      \draw (0,0) -- ++(1.5,-2) node{$\bullet$} node[below]{$s_p$} 
      -- ++(-3,0) node[pos=0.3,below]{$\ldots$} node[near end,below]{$\ldots$} node{$\bullet$} node[below]{$s_1$}
      -- cycle;
      \draw (0,0) -- ++(0.2,-0.5) 
      -- ++(-0.8,-0.7) node[right=0.6em]{$\dpath{\vec\rho}$} 
      -- (0,-2) node{$\bullet$} node[below]{$s_l$};
    \end{tikzpicture}
  \end{center}
  \caption{\label{fig:cca-alternate}Shape of a decryption oracle term $C[\vec g \diamond (s_i)_{i\le p}]$. The upper part is composed of conditionals (the guards), and the lower part ($(s_i)_{i\le p}$) are the result of the oracle call.}
\end{wrapfigure}
where $s \equiv t\left[(\alpha_{i})_{i \le n},(\dec_j)_{j \le m}\right]$, the terms $(\alpha_i)_{i \le n}$ are encryption oracle calls, and the terms $(\dec_j)_{j \le m}$ are decryption oracle calls (not necessary with the same key) which are themselves of the same form. We would like to have all guards at the top-level, not only the top-most call to the decryption oracle but also the guards of the inner calls $(\dec_j)_{j \in m}$. 

This can be easily achieved by repeatedly pulling out the inner guards. We require smaller guards to be higher (where $s$ is smaller than $t$ if $s \in \st(t)$ and $s \ne t$), and as we want to have a unique way of guarding a decryption we would extend the strict subterm order into an arbitrary total ordering on ground conditionals~$\succ_g$. The problem is that we want to use the ordering for terms on the left and on the right of $\sim$, but the guard will not be the same on the left and on the right (since they have different encryptions). As there is no way to have a total ordering on ground terms that give the same order for ``equivalent'' conditionals on the left and right side of $\sim$ (i.e. conditionals that only differ by their encryptions), we have to use a slightly different approach: instead of a total order on ground conditionals, we let $\succ_g$ be a total order on conditionals in $\mathcal{T}(\sig,\encvar)$. 

\begin{definition}
  We say that a decryption $s \equiv \dec(t,\sk)$ is well-guarded in term $u$ under keys $\keys$ (where $\sk \in \keys$) and encryptions $\encs = \{ \alpha_i  \mid i\}$ if $u$ is of the form given in Fig.~\ref{fig:cca-alternate}, where:
  \begin{itemize}
  \item Let $D$ be the set of decryptions under keys in $\keys$ appearing in subterms of $s$ when removing the encryptions~$\encs$:
    \[
      \mathcal{D} \, = \, \{\dec(v,\key_v) \in \st(s) \mid \key_v \in \keys \wedge \dec(v\{0 / \encs \},\key_v) \in \st(s\{0 / \encs \})\}
    \]
    Moreover we decompose $\mathcal{D}$ into disjoint sets $\mathcal{D}_1,\dots,\mathcal{D}_q$ where for every $i < j$, decryptions in $\mathcal{D}_j$ are not subterms of decryptions in $\mathcal{D}_i$. In other words $\mathcal{D}_1$ contains the smallest decryptions, $\mathcal{D}_2$ contains decryptions that are built using decryptions in $\mathcal{D}_1$ etc ... Formally:
    \[
      \forall i < j,\,\forall v \in \mathcal{D}_i, \forall w \in \mathcal{D}_j,\, w \not \in \st(v)
    \]

    We let $\dpath{\vec{\rho}} =  \dpath{\vec\rho}_1,\dots, \dpath{\vec \rho}_q$ where for all $1 \le a \le q$, $\dpath{\vec{\rho}}_a$ are the guards corresponding to decryptions in $\mathcal{D}_a$, knowing that we are in the branch $ \dpath{\vec \rho}_1,\dots, \dpath{\vec \rho}_{a-1}$. To do this we require that $ \dpath{\vec \rho}_a$ contains one guard $\eq{t_i\encmap^a}{\alpha_j}$ for every $\dec(t_i,\sk(\nonce_i)) \in \mathcal{D}_a$ with $\sk(\nonce_i) \in \keys$ and $\alpha_j \equiv \enc{\_}{\pk(\nonce_i)}{\_} \in \st(t_i)$ (with $\alpha_j \in \encs$), where $\encmap^a$ is the $\encs$-quasi substitution that replaces every bad call to the decryption oracles $d$ in $ \dpath{\vec \rho}_1,\dots, \dpath{\vec \rho}_{a-1}$ by~$\zero(d)$. We call an $\mathcal{\encvar}$-quasi substitution a function $\encmap$ that does not ``go below'' terms in $\mathcal{\encvar}$ (i.e. $\forall v \in \mathcal{\encvar}, v\encmap \equiv v$) but otherwise behave as a substitution, and we let $\encmap^a$ be the $\encs$-quasi substitution defined as:
    \[
      \encmap^a = \encmap^{a-1}\,\{ 0(d) / \underbrace{\dec(t_i\encmap^{a-1},\sk(\nonce_i))}_{d} \mid \exists a' < a,\, \eq{d}{\alpha_j} \text{ appears positively in } \dpath{\vec \rho}_{a'}  \}
    \]
    where a guard is said to appear \emph{positively} in $ \dpath{\vec \rho}_{a'}$ if it appears in $ \dpath{\vec \rho}_{a'}$ and the path continues in the \textsf{then} branch of this guard.

  \item We require that ${{\vec \rho}} \{ x_i/\alpha_i \mid \alpha_i \in \mathcal{E} \}$ is in increasing order for $\succ_g$.
  \item For every $l$, the term $s_l \equiv s\, \encmap^{q+1}$.
  \end{itemize}
\end{definition}

\begin{example} Consider the following decryption oracle call $t$ (we did not write the arguments of the $\zero$ functions for simplicity):
  \begin{alignat*}{2}
    t \equiv \ite{b}{&\zero(\_)\\}
    {&\dec\left(g_1\left(
          \begin{alignedat}{2}
            \ite{\eq{g_0(\enc{A}{\pk}{\nonce_r})}{\enc{A}{\pk}{\nonce_r}}}{&\zero(\_)\\}
            {
              &\dec(g_0(\enc{A}{\pk}{\nonce_r}),\sk))
            }
          \end{alignedat}
        \right),\sk\right)}
  \end{alignat*}
  where $b$ is the conditional:
  \[
    b \equiv 
    \textsf{EQ}\left(g_1\left(
        \begin{alignedat}{2}
          \ite{\eq{g_0(\enc{A}{\pk}{\nonce_r})}{\enc{A}{\pk}{\nonce_r}}}{&\zero(\_)\\}
          {
            &\dec(g_0(\enc{A}{\pk}{\nonce_r}),\sk))
          }
        \end{alignedat}\right)
      \,,\,\enc{A}{\pk}{\nonce_r}\right)
  \]
  Then we can rewrite $t$ by pulling the internal guard to the top level, and simplifying below accordingly. This yield the following term:
  \begin{alignat*}{2}
    t =_R
    \ite{\eq{g_0(\enc{A}{\pk}{\nonce_r})}{\enc{A}{\pk}{\nonce_r}}}
    {&
      \begin{alignedat}[t]{2}
        \ite{\eq{g_1(\zero(\_))}{\enc{A}{\pk}{\nonce_r}}}{&\zero(\_)\\}
        {&\dec\left(g_1\left(
              {\zero(\_)}
            \right),\sk\right)}
      \end{alignedat}
      \\}
    {&
      \begin{alignedat}[t]{2}
        \ite{\eq{
            g_1\left(\dec(g_0(\enc{A}{\pk}{\nonce_r}),\sk))\right)
          }{\enc{A}{\pk}{\nonce_r}}}{&\zero(\_)\\}
        {&\dec\left(g_1\left(
              \dec(g_0(\enc{A}{\pk}{\nonce_r}),\sk))
            \right),\sk\right)}
      \end{alignedat}
    }
  \end{alignat*}
\end{example}

\begin{definition} For any finite set of key pairs $\keys$, we let $R_{\CCA_e}^\keys$ be the binary relation having the same definition than $R_{\CCA_b}^\keys$, apart for the third case that we replace by:
  \begin{enumerate}
    \setcounter{enumi}{2}
  \item Let $\sk \in \keys$, $\pk$ the corresponding public key, $C$ be an if-context and $z$ be a fresh variable:
    \begin{equation*}
      \left(\left(\phi,u\right),\encvar,\decvar \cup \{z\},\randmap, \encmap,\decmap\cup \{z \mapsto u\}  \right) 
      R_{\CCA_e}^\keys  \left(\left(\psi,v\right),\encvar,\decvar \cup \{z\},\randmap', \encmap',\decmap'\cup \{z \mapsto v\}\right)
    \end{equation*}
    if $\exists \vec g,(s_a)_{a \le p} \in \mathcal{T}(\sig,\encvar)$ such that:\\[1em]
    \(
    \displaystyle
    \left\{ 
      \begin{array}{ll}
        \bullet & (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_e}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')\\
        \bullet &  u \equiv C[\vec g\encmap \diamond (s_a\encmap)_{a \le p}] \text{ and } v \equiv C[\vec g\encmap' \diamond (s_a\encmap')_{a \le p}]\\
        \bullet & \text{the right-most element $s_p$ is of the form } t_p \equiv \dec(t_p,\sk)\\
        \bullet & \dec(t_p\encmap,\sk) \text{ is well-guarded in } u \text{ under } (\keys,\encvar\encmap)\\
        \bullet & \dec(t_p\encmap',\sk) \text{ is well-guarded in } v \text{ under } (\keys,\encvar\encmap')\\
        \bullet & \nodec(\keys;t_p) \text{ and }\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)
      \end{array}
    \right.
    \)
  \end{enumerate}

  We let CCA$_e$ be the set of unitary axioms $\phi \sim \psi$ such that there exist $\keys,\encvar,\decvar,\randmap,\randmap',\encmap,\encmap'$ with
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_e}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
\end{definition}

\begin{proposition}
  For all instance of $R_{\CCA_b}^\keys$:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_b}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  there exists $\tilde \phi,\tilde \psi,\tilde \encmap,\tilde \decmap,\tilde \encmap',\tilde \decmap'$ such that:
  \begin{itemize}
  \item $\tilde \phi =_{R} \phi$ and $\tilde \psi =_{R} \psi$.
  \item $\forall x \in \encvar, x\tilde \encmap =_{R} x \encmap$ (same for $\encmap'$) and $\forall x \in \decvar, x\tilde \decmap =_{R} x \decmap$ (same for $\decmap'$).
  \item This is an instance of  $R_{\CCA_e}^\keys$:
    \[
      (\tilde \phi,\encvar,\decvar,\randmap,\tilde \encmap,\tilde \decmap) R_{\CCA_e}^\keys (\tilde \psi,\encvar,\decvar,\randmap',\tilde \encmap',\tilde \decmap')
    \]
  \end{itemize}
\end{proposition}

\begin{proofatend}
  We prove this by induction on the definition of $R_{\CCA_b}^\keys$. The only interesting case is the third case, hence take:
  \begin{multline*}
    \left(\left(\phi,\elses(l,\dec(u,\sk))\right),\encvar,\decvar \cup \{z\},\randmap, \encmap,\decmap\cup \{z \mapsto \elses(l,\dec(u,\sk))\}  \right) \\
    R_{\CCA_b}^\keys  \left(\left(\psi,\elses(l',\dec(v,\sk))\right),\encvar,\decvar \cup \{z\},\randmap', \encmap',\decmap'\cup \{z \mapsto \elses(l',\dec(v,\sk))\}\right)
  \end{multline*}
  where $\sk \in \keys$, $\pk$ is the corresponding public key, $\{x_1,\dots,x_n\}$ is the set of variables $x \in \encvar$ such that $x\encmap$ is an encryption using public-key $\pk$ and $z$ is a fresh variable. By definition of $R_{\CCA_b}^\keys$ we there exists $t \in \mathcal{T}(\sig,\encvar \cup \decvar)$ such that:
  \begin{itemize}
  \item $ (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_b}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$
  \item $u \equiv t\encmap\decmap$ and $v \equiv t\encmap'\decmap'$
  \item $ l \equiv \left(\eq{u}{x_1\encmap},\dots,\eq{u}{x_n\encmap}\right)$ and $ l' \equiv \left(\eq{v}{x_1\encmap'},\dots,\eq{v}{x_n\encmap'}\right)$
  \item $\nodec(\keys;t)$ and $\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$
  \end{itemize}
  By induction hypothesis we have there exists $\tilde \phi,\tilde \psi,\tilde \encmap,\tilde \decmap,\tilde \encmap',\tilde \decmap'$ such that:
  \begin{itemize}
  \item $\tilde \phi =_{R} \phi$ and $\tilde \psi =_{R} \psi$.
  \item $\forall x \in \encvar, x\tilde \encmap =_{R} x \encmap$ (same for $\encmap'$) and $\forall x \in \decvar, x\tilde \decmap =_{R} x \decmap$ (same for $\decmap'$).
  \item This is an instance of  $R_{\CCA_e}^\keys$:
    \[
      (\tilde \phi,\encvar,\decvar,\randmap,\tilde \encmap,\tilde \decmap) R_{\CCA_e}^\keys (\tilde \psi,\encvar,\decvar,\randmap',\tilde \encmap',\tilde \decmap')
    \]
  \end{itemize}
  Since $\encvar \cap \decvar = \emptyset$, and since for all $x \in \encvar$, the term $x\encmap$ is ground we know that $t\encmap\decmap \equiv t\decmap\encmap$. We let $\{z_1,\dots,z_m\}$ be the set of variable $z \in \decvar \cap \var(t)$. By induction hypothesis we know that for all $1 \le i \le m$, there exits $C_i,\vec g_i, (s_a^i)_{a \in A_i}$ such that:
  \[
    z_i \decmap =_R z_i \tilde \decmap \equiv C_i[\vec g_i \diamond (s_a^i)_{a \in A_i}]\tilde \encmap
  \]

  We let $\vec g$ be the list of all conditionals in $\{ b \mid \exists i, b \in \vec g_i\}$ ordered by $\succ_g$, and we let $C$ be the if-context such that the conditional at depth $k$ in $C[\vec g \diamond \_]$ is the $k$-th element of $\vec g$. Then we know that there exits substitutions $(\tilde \decmap_{\dec}^a)_{a \in A}$ with domain $\{z_1,\dots,z_m\}$ such that:
  \[
    t \tilde \decmap\tilde \encmap =_R C[\vec g \diamond (t\tilde \decmap_{\dec}^a)_{a \in A}]\tilde \encmap
  \]
  where the substitution $\tilde \decmap_{\dec}^a$ is defined as follows: let $\dpath{\vec \rho_a}$ be the directed path of conditionals occurring from the root of $C$ to leave $a$. We know that $\vec \rho_a \equiv \vec g$ (recall that $\vec \rho_a$ is the list of conditionals only extracted from $\dpath{\vec \rho_a}$), therefore for all $1 \le i \le m$, there exists $a_i \in A_i$ such that the directed path of conditionals $\dpath{\vec \rho_{a_i}}$ occurring from the root of $C_i[\vec g_i \diamond \_]$ to leave $a_i$ is included in $\dpath{\vec \rho_a}$ (here we talk about inclusion of directed paths, hence the directions are taken into account). We then let $z_i\tilde \decmap_{\dec}^a \equiv s_a^i$.

  We let $\vec g_2$ be list of conditionals obtained by extending $\vec g$ on the right with:
  \[
    \bigcup_{a \in A}\left(\eq{t\tilde \decmap_{\dec}^a}{x_1},\dots,\eq{t\tilde \decmap_{\dec}^a}{x_n}\right)
  \]
  Moreover we require that the new conditionals are ordered by $\succ_g$. Observe that:
  \begin{align*}
    &&&\elses\left((\eq{u}{x_1\encmap},\dots,\eq{u}{x_n\encmap}),\dec(u,\sk)\right)\\
    &\equiv&&\elses\left((\eq{t\decmap\encmap}{x_1\encmap},\dots,\eq{t\decmap\encmap}{x_n\encmap}),\dec(t\decmap\encmap,\sk)\right)\\
    &=_R&&\elses\left((\eq{t\tilde \decmap\tilde \encmap}{x_1\tilde \encmap},\dots,\eq{t\tilde \decmap\tilde \encmap}{x_n\tilde \encmap}),
    \dec(t\tilde \decmap\tilde \encmap,\sk)\right)\\
    &=_R&&\elses\left((\eq{C[\vec g \diamond (t\tilde \decmap_{\dec}^a)_{a \in A}]\tilde \encmap}{x_1\tilde \encmap},\dots,\eq{C[\vec g \diamond (t\tilde \decmap_{\dec}^a)_{a \in A}]\tilde \encmap}{x_n\tilde \encmap}),
    \dec(C[\vec g \diamond (t\tilde \decmap_{\dec}^a)_{a \in A}]\tilde \encmap,\sk)\right)\\
    &=_R&&
    C\left[\vec g \diamond
      \left(
        \elses\left(
          (\eq{t\tilde \decmap_{\dec}^a\tilde \encmap}{x_1\tilde \encmap},
          \dots,
          \eq{t\tilde \decmap_{\dec}^a\tilde \encmap}{x_n\tilde \encmap}
        \right),
        \dec(t\tilde \decmap_{\dec}^a\tilde \encmap,\sk)
      \right)
    \right]\\
    &\equiv&&
    C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap
  \end{align*}
  where $C_2$ is an if-context, $A_2 = A \times \{1,\dots,n+1\}$ and for all $(a,j) \in A_2$:
  \[
    s_{(a,j)} \equiv
    \begin{cases}
      \dec\left(t\tilde \decmap_{\dec}^a,\sk\right) & \text{ if } j = n+1\\
      \zero\left(\dec(t\tilde \decmap_{\dec}^a,\sk)\right) & \text{ otherwise}
    \end{cases}
  \]
  Let $s_p$ be the right-most element of $(s_c)_{c \in A_2}$. One can then check that $\dec(s_p\tilde \encmap,\sk)$ is well-guarded in $C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap$ under $(\encvar\tilde \encmap,K)$. Doing the same reasoning on $t'$, we get that:
  \[
    \elses\left((\eq{u'}{x_1\encmap'},\dots,\eq{u'}{x_n\encmap'}),\dec(u',\sk)\right) =_E
    C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap'
  \]
  and that $\dec(s_p\tilde \encmap',\sk)$ is well-guarded in $C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap$ under $(\encvar\tilde \encmap',K)$. Moreover we know that $\nodec(\keys;t)$, and that:
    \begin{equation}\label{eq:cca-syntact}
      (\tilde \phi,\encvar,\decvar,\randmap,\tilde \encmap,\tilde \decmap) R_{\CCA_e}^\keys (\tilde \psi,\encvar,\decvar,\randmap',\tilde \encmap',\tilde \decmap')
    \end{equation}
    From Equation~\eqref{eq:cca-syntact} we get that $\hiddenr(\encvar\randmap \cup \encvar\randmap';\tilde \phi,\tilde \psi)$, and using the fact that $\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$ we can check that $\hiddenr(\encvar\randmap \cup \encvar\randmap';C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap,C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap')$. Hence we have:
    \[
      \hiddenr(\encvar\randmap \cup \encvar\randmap';\tilde \phi,C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap,\tilde \psi,C_2\left[\vec g_2 \diamond (s_c)_{c \in A_2} \right]\tilde \encmap')
    \]
  Which concludes this proof
\end{proofatend}

\begin{definition}
  We let $R_{\CCA_d}^\keys$ be the restriction of $R_{\CCA_e}^\keys$ to the instances where all conditionals appearing in decryptions are either guards or ``below'' encryptions.  Formally $R_{\CCA_d}^\keys$ is the restriction of $R_{\CCA_e}^\keys$ to the instances:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_e}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  where for all $x \in \decvar$, $x\decmap$ is of the form $C[\vec g\encmap \diamond (s_a\encmap)_{a \le p}]$ (with $C$ and if-context and $\vec g,(s_a)_{a \le p} \in \mathcal{T}(\sig,\encvar)$) and  the right-most element $s_p$ is \emph{if-free}.

  We let CCA$_d$ be the set of unitary axioms $\phi \sim \psi$ such that there exist $\keys,\encvar,\decvar,\randmap,\randmap',\encmap,\encmap'$ with
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_d}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
\end{definition}

\begin{proposition}
  For all instance $\vec u \sim \vec u'$ of CCA$_{c}$, there exists a proof of $\vec u \sim \vec u'$ using rules $R + CS_{\textsf{gen}} + \text{CCA}_d$, where $CS_{\textsf{gen}}$ is the unrestricted version of $CS$.
\end{proposition}

\begin{proof}
  \todo{TODO}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ms"
%%% End:


==> detailled-cca.tex <==
% This file contains a detailled description of 3 version of the CCA axiom, which I decided not to include in the paper.

\subsection{Length in The Logic and the \cca Axiom}
\input{length}

\subsection{\cca Axiom}
\label{section:cca-axiom}
\begin{proofatendsection}
\end{proofatendsection}
\todo{We never explained how the alpha renaming of names works: should change \cca to allow renaming up to encryption oracle calls}

\todo{Add lengths in this proof}

In this appendix we are going to define and prove correct an axiom for an $\textsc{ind-cca}_2$ encryption scheme.

Consider the following multi-users $\textsc{ind-cca}_2$ game: the adversary receives $n$ public-keys. For each of these keys $\pk_i$ he has access to a left-right oracle $LR_{\pk_i}$, that takes two messages $m_0,m_1$ as input and returns $\{m_b\}_{\pk_i}^{\nonce_r}$, where $b$ is internal random bit uniformly drawn at the beginning by the challenger (the same $b$ is used for all $LR$ oracles) and $\nonce_r$ is a fresh nonce. Moreover, for all key pairs $(\pk_i,\sk_i)$, the adversary has access to an $\sk_i$ decryption oracle, but cannot call the $\sk_i$ decryption oracle on a cipher-text returned by $LR_{\pk_i}$. The advantage of an adversary against this game and the multi-user $\textsc{ind-cca}_2$ security are defined as usual.

It is known that an $\textsc{ind-cca}_2$ secure game is also multi-users $\textsc{ind-cca}_2$ secure (see~\cite{musu}), so we will allow multiple key pairs to appear in the \cca axiom, and multiple encryptions over different terms using the same public key (each encryption corresponds to one call to the $LR$ oracle).


\paragraph{} If we want the following to hold in any computational model
\[
  \dec\left(t\left[\{u_1\}_{\pk}^{\nonce_r^1},\dots,\{u_n\}_{\pk}^{\nonce_r^n}\right],\sk\right) \sim \dec\left(t\left[\{v_1\}_{\pk}^{\nonce_r'^1},\dots,\{v_n\}_{\pk}^{\nonce_r'^n}\right],\sk\right)
\]

then we need to make sure that $t[\{u_1\}_{\pk}^{\nonce_r^1},\dots,\{u_n\}_{\pk}^{\nonce_r^n}]$ is different from all $\{u_i\}_{\pk}^{\nonce_r^i}$ and that $t[\{v_1\}_{\pk}^{\nonce_r'^1},\dots,\{v_n\}_{\pk}^{\nonce_r'^n}]$ is different from all $\{v_i\}_{\pk}^{\nonce_r'^i}$. This is done by introducing all the unwanted equalities in $\ite{}{}{}$ tests and making sure that we are in the else branch of all these tests, so as to have a ``safe call'' to the decryption oracle. Moreover the adversary is allowed to use values obtained from previous calls to the decryption oracle in future calls.

This lead us to the following definition:
\begin{definition} We define the function $\elses$ by induction:
  \begin{align*}
    &\elses(\emptyset, x) \equiv x\\
    &\elses\left((\eq{a}{b}) :: \Gamma, x\right) \equiv \ite{\eq{a}{b}}{\elses(\Gamma,x)}{\zero(x)}
  \end{align*}
\end{definition}

\begin{example}
  Let $u \equiv t[\{v_1\}_{\pk}^{\nonce_r^1},\{v_2\}_{\pk}^{\nonce_r^2}]$. Then:
  \begin{multline*}
    \elses\left(\left(\eq{u}{\{v_1\}_{\pk}^{\nonce_r^1}},\eq{u}{\{v_2\}_{\pk}^{\nonce_r^2}}\right),\dec(u,\sk)\right) \equiv\\
    \ite{\eq{u}{\{v_1\}_{\pk}^{\nonce_r^1}}}{\zero(\dec(u,\sk))}{\ite{\eq{u}{\{v_2\}_{\pk}^{\nonce_r^2}}}{\zero(\dec(u,\sk))}{\dec(u,\sk)}}
  \end{multline*}
  This term represent a ``safe call'' to the decryption oracle.
\end{example}


\paragraph{} We will use the following notations: for any finite set $\keys$ of valid private keys, $\keys \decpos \vec u$ holds if for all $\sk \in \keys$, the secret key $\sk$ appears only in decryption position in $\vec u$; $\fresh{\vec{u}}{\vec v}$ denotes the fact that no term of $\vec u$ is a subterm of a term of $\vec v$; $\nodec(\keys,\vec u)$ denotes that for all $\sk(\nonce) \in \keys$, the only occurrences of $\nonce$ are in subterms $\pk(\nonce)$;  $\hiddenr(\vec r;\vec u)$ denotes that for all $\nonce_r \in \vec r$, $\nonce_r$ appears only in encryption randomness position and is not used with two distinct plaintexts.

We are now going to define by induction the \cca axiom. In order to do this we will define by induction a binary relation $R_{\CCA_a}^\keys$ where $K$ will be the finite set of private keys used in the terms (corresponding to the public keys sent by the challenger). Before defining formally this relation let us give some intuition to $(\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$: $\phi$ and $\psi$ are the vectors of terms that are indistinguishable for a PPTM ($\phi \sim \psi$ will be a valid application of \cca); $\encvar$ and $\decvar$ will be two disjoint sets of variables; $\randmap$ (resp. $\randmap'$) will be a substitution of domain $\encvar$ and whose codomain is the set of encryption randomnesses in $\phi$ (resp. $\psi$) used to encrypt different messages in $\phi$ and in $\psi$; $\encmap$ (resp. $\encmap'$) will be a substitution of domain $\encvar$ and whose codomain is the set of encryption oracle calls in $\phi$ (resp. $\psi$) that are different in $\phi$ and in $\psi$; $\decmap$ (resp. $\decmap'$) will be a substitution of domain $\decvar$ and whose codomain is the set of decryption oracle calls in $\phi$ (resp. $\psi$).


\begin{definition} For any finite set of key pairs $\keys$, we define the binary relation $R_{\CCA_a}^\keys$ by induction as follows:
  \begin{enumerate}
  \item \textbf{No Call to the Oracles:} if $\keys \decpos \phi$ then $(\phi,\emptyset,\emptyset,\emptyset,\emptyset,\emptyset) R_{\CCA_a}^\keys (\phi,\emptyset,\emptyset,\emptyset,\emptyset,\emptyset)$

  \item \textbf{Encryption Case:} $x$ a fresh variable that does not appear in $\encvar \cup \decvar$, $\sk \in \keys$ and $\pk$ the corresponding public key:
    \begin{multline*}
      \left((\phi,\{u\}_{\pk}^{\nonce_r}),\encvar \cup \{x\},\decvar,\randmap \cup \{x \mapsto \nonce_r\}, \encmap \cup \{x \mapsto \{u\}_{\pk}^{\nonce_r}\} ,\decmap\right) \\R_{\CCA_a}^\keys  \left((\psi,\{v\}_{\pk}^{\nonce_r'}),\encvar \cup \{x\},\decvar,\randmap' \cup \{x \mapsto \nonce_r'\}, \encmap' \cup \{x \mapsto \{v\}_{\pk}^{\nonce'_{r}}\} ,\decmap'\right)
    \end{multline*}
    if the following conditions hold:
    \begin{itemize}
    \item $(\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$
    \item $\keys \decpos u,v$
    \item $\fresh{\nonce_r,\nonce_r'}{\phi,u,\psi,v} \text{ and } \hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$
    \end{itemize}
    
  \item \textbf{Decryption Case:} Let $\sk \in \keys$, $\pk$ the corresponding public key, and $\{x_1,\dots,x_n\}$ be the set of variables $x \in \encvar$ such that $x\encmap$ is an encryption using public-key $\pk$ and $z$ be a fresh variable:
    \begin{multline*}
      \left(\left(\phi,\elses(l,\dec(u,\sk))\right),\encvar,\decvar \cup \{z\},\randmap, \encmap,\decmap\cup \{z \mapsto \elses(l,\dec(u,\sk))\}  \right) \\
      R_{\CCA_a}^\keys  \left(\left(\psi,\elses(l',\dec(v,\sk))\right),\encvar,\decvar \cup \{z\},\randmap', \encmap',\decmap'\cup \{z \mapsto \elses(l',\dec(v,\sk))\}\right)
    \end{multline*}
    if there exists $t \in \mathcal{T}(\sig,\encvar \cup \decvar)$ such that the following conditions hold:
    \begin{itemize}
    \item $(\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$
    \item $ u \equiv t\encmap\decmap$ and $v \equiv t\encmap'\decmap'$
    \item $l \equiv \left(\eq{u}{x_1\encmap},\dots,\eq{u}{x_n\encmap}\right)$
    \item $l' \equiv \left(\eq{v}{x_1\encmap'},\dots,\eq{v}{x_n\encmap'}\right)$
    \item $\nodec(\keys;t) \text{ and } \hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$
    \end{itemize}
  \end{enumerate}
\end{definition}

\begin{definition}
  CCA$_a$ is the set of unitary axioms $\phi \sim \psi$ such that there exist $\keys,\encvar,\decvar,\randmap,\randmap',\encmap,\encmap'$ such that we have:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
\end{definition}

\begin{proposition}
  All formulas in $\CCA_a$ are computationally valid if the encryption scheme is $\textsc{ind-cca}_2$ secure.
\end{proposition}

\begin{proofatend}
  Let \cmodel be a computational model where the encryption and decryption symbol are interpreted as an $\textsc{ind-cca}_2$ secure encryption scheme. Let $\phi \sim \psi$ be an instance of \cca such that $\llbracket \phi \rrbracket_{\cmodel} \not \approx_{\cmodel} \llbracket \psi \rrbracket_{\cmodel} $ i.e. there is a PPTM $\mathcal{A}$ that has a non-negligible advantage of distinguishing these two distributions.

  Since $\phi \sim \psi$ is an instance of \cca we know that there exists $\keys,\encvar,\decvar,\randmap,\encmap,\randmap',\encmap',\decmap,\decmap'$ such that:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]

  We are going to build from $\phi$ and $\psi$ a winning attacker against the multi-user $\textsc{ind-cca}_2$ game. This attacker has access to a $LR$ oracle and a decryption oracle for all keys in $\keys$. We are going to build by induction on $R_{\CCA_a}^\keys$ a algorithm $\mathcal{B}$ that samples from $\llbracket \phi \rrbracket_{\cmodel}$ or $\llbracket \psi \rrbracket_{\cmodel}$ (depending on the oracles internal bit). The algorithm $\mathcal{B}$ uses a memoisation technique: it builds a store whose keys are subterms of $\phi, \psi$ already encountered and variable in $\encvar \cup \decvar$, and values are elements of the \cmodel domain.
  \begin{enumerate}
  \item $(\phi,\emptyset,\emptyset,\emptyset,\emptyset,\emptyset) R_{\CCA_a}^\keys (\phi,\emptyset,\emptyset,\emptyset,\emptyset,\emptyset)$: for all terms $t$ in the vector $\phi$, $\mathcal{B}$ samples from $\llbracket t \rrbracket_{\cmodel}$ by induction as follows:
    \begin{itemize}
    \item if $t$ is in the store then $\mathcal{B}$ returns its value.
    \item nonce $\nonce$: $\mathcal{B}$ draws $\nonce$ uniformly at random and stores the drawn value. 

      Remark that $\keys \decpos \phi$ ensures us that $\nonce$ is not a secret key $\sk$ appearing in $\keys$, which we could not compute. If it is a public key $\pk$,  either the corresponding secret key $\sk$ is such that $\sk \in \keys$ and the challenger sent us a random sample from $\llbracket \pk \rrbracket_{\cmodel}$, or $\sk$ does not appear in $\keys$ and then $\mathcal{B}$ can draw the corresponding key pair itself.

    \item $f(t_1,\dots,t_n)$:
      \begin{itemize}
      \item If $f$ is not a decryption then $\mathcal{B}$ inductively samples the function arguments $\left(\llbracket t_1 \rrbracket_{\cmodel},\dots,\llbracket t_1 \rrbracket_{\cmodel} \right)$ and then $\llbracket f \rrbracket_{\cmodel} \left(\llbracket t_1 \rrbracket_{\cmodel},\dots,\llbracket t_1 \rrbracket_{\cmodel} \right)$.

      \item If $f$ is a decryption over $\sk$ appearing in $\keys$ then $\mathcal{B}$ calls the $\sk$ decryption oracle (no call were made to the $LR$ oracles yet, so we can call the decryption oracles on any value).
      \end{itemize}
      In both cases $\mathcal{B}$ stores the value at the key $f(t_1,\dots,t_n)$.
    \end{itemize}

  \item Encryption case:
    \begin{multline*}
      \left((\phi,\{u\}_{\pk}^{\nonce_r}),\encvar \cup \{x\},\decvar,\randmap \cup \{x \mapsto \nonce_r\}, \encmap \cup \{x \mapsto \{u\}_{\pk}^{\nonce_r}\} ,\decmap\right) \\R_{\CCA_a}^\keys  \left((\psi,\{v\}_{\pk}^{\nonce_r'}),\encvar \cup \{x\},\decvar,\randmap' \cup \{x \mapsto \nonce_r'\}, \encmap' \cup \{x \mapsto \{v\}_{\pk}^{\nonce_r'}\} ,\decmap'\right)
    \end{multline*}

    Since we have $\fresh{\nonce_r,\nonce_r'}{\phi,u,\psi,v}$ we know that the toplevel terms do not appear in the store. We start by observing that if the challenger internal bit is $0$ then for all $w$:
    $$LR_{\pk}(\llbracket u \rrbracket_{\cmodel},\llbracket v \rrbracket_{\cmodel}) = LR_{\pk}(\llbracket u \rrbracket_{\cmodel},w)$$

    Similarly if the challenger internal bit is $1$ then for all $w$:
    $$LR_{\pk}(\llbracket u \rrbracket_{\cmodel},\llbracket v \rrbracket_{\cmodel}) = LR_{\pk}(w,\llbracket v \rrbracket_{\cmodel})$$

    $\mathcal{B}$ will sample two values $\alpha, \beta$ such that if the challenger internal bit is $0$ then $\alpha$ is sampled from $\llbracket u \rrbracket_{\cmodel}$ and if the challenger internal bit is $1$ then $\beta$ is sampled from $\llbracket v \rrbracket_{\cmodel}$. Therefore whatever the challenger internal is bit, $LR_{\pk}(\alpha,\beta)$ is sampled from $LR_{\pk}(\llbracket u \rrbracket_{\cmodel},\llbracket v \rrbracket_{\cmodel})$:
    \begin{itemize}
    \item $\alpha$ is sampled from $\llbracket u \rrbracket_{\cmodel}$ using the case 1 algorithm except for decryption $\dec(w,\sk')$ where $\sk'$ appears in $\keys$. In that case $\mathcal{B}$ inductively samples $\gamma$ from $\llbracket w \rrbracket_{\cmodel}$. If $\gamma$ is \emph{not} equal to the cipher returned by a previous call $LR_{\pk'}(\delta,\epsilon)$ then $\mathcal{B}$ can call the $\sk'$ decryption oracle, otherwise $\mathcal{B}$ returns $\delta$. Remark that if the internal bit is $0$ then $\delta$ is the decryption of $\gamma$ by $\sk'$.

    \item $\beta$ is sampled from $\llbracket v \rrbracket_{\cmodel}$ using the case 1 algorithm except for decryption $\dec(w,\sk')$ where $\sk'$ appears in $\keys$. In that case $\mathcal{B}$ inductively samples $\gamma$ from $\llbracket w \rrbracket_{\cmodel}$. If $\gamma$ is \emph{not} equal to the cipher returned by a previous call $LR_{\pk'}(\delta,\epsilon)$ then $\mathcal{B}$ can call the $\sk'$ decryption oracle, otherwise $\mathcal{B}$ returns $\epsilon$. Remark that if the internal bit is $1$ then $\epsilon$ is the decryption of $\gamma$ by $\sk'$.
    \end{itemize}

    The condition $\keys \decpos u,v$ ensures that no secret key from $\keys$ appears anywhere else than in decryption position, and the two conditions $\fresh{\nonce_r,\nonce_r'}{\phi,u,\psi,v}$ and $\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$ ensure that all randomnesses used by the challenger $LR$ oracles do not appear anywhere else than in encryption randomness position for the corresponding $LR$ oracle call.

    We store the result of the $LR$ oracle call at key $x$.
  \item Decryption case:
    \begin{multline*}
      \left(\left(\phi,\elses(l,\dec(u,\sk))\right),\encvar,\decvar \cup \{z\},\randmap, \encmap,\decmap\cup \{z \mapsto \elses(l,\dec(u,\sk))\}  \right) \\R_{\CCA_a}^\keys  \left(\left(\psi,\elses(l',\dec(v,\sk))\right),\encvar,\decvar \cup \{z\},\randmap', \encmap',\decmap'\cup \{z \mapsto \elses(l',\dec(v,\sk))\}\right)
    \end{multline*}

    We know that $u \equiv t\encmap\decmap$ and $v \equiv t\encmap'\decmap'$. Moreover it is easy to check that $\mathcal{B}$ inductive definition is such that $\mathcal{B}$ store has a value associated with every variable in $\encvar \cup \decvar$ and that, if $x \in \encvar$, then the store value of $x$ is either sampled from $\llbracket x\encmap \rrbracket_{\cmodel}$ or from $\llbracket x\encmap' \rrbracket_{\cmodel}$ (depending on the challenger internal bit), and that if $x \in \decvar$ then the store value of $x$ is either sampled from $\llbracket x\decmap \rrbracket_{\cmodel}$ or from $\llbracket x\decmap' \rrbracket_{\cmodel}$ (depending on the challenger internal bit).

    $\mathcal{B}$ uses the case 1 algorithm to sample $\gamma$ from $\llbracket t\encmap\decmap \rrbracket$ or $\llbracket t\encmap'\decmap' \rrbracket$ depending on the challenger internal bit. The variable case was dealt with in the previous paragraph, $\nodec(\keys;t)$ ensures us that no call to the decryption oracles are needed and $\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$ guarantee that the randomness drawn by the challenger for $LR$ oracle encryption do not appear in $t$.

    Observe that all calls to $LR_{\pk}$ have been stored at keys $x_1,\dots,x_n$. Hence if $\gamma$ is equal to any of the value stored at keys $x_1,\dots,x_n$ then $\mathcal{B}$ return $0$, otherwise $\mathcal{B}$ can call the $\sk$ decryption oracle on $\gamma$.

    We store the result at key $z$.
  \end{enumerate}

  \paragraph{} The attacker against the multi-user $\textsc{ind-cca}_2$ game simply returns $\mathcal{A}(\mathcal{B})$. Since $\mathcal{B}$ samples either from $\llbracket \phi \rrbracket_{\cmodel}$ if $b = 0$ or from  $\llbracket \psi \rrbracket_{\cmodel}$ if $b = 1$, and since $\mathcal{A}$ has a non-negligible advantage of distinguishing  $\llbracket \phi \rrbracket_{\cmodel}$ from  $\llbracket \psi \rrbracket_{\cmodel}$ we know that the attacker has a non-negligible advantage against the multi-user $\textsc{ind-cca}_2$ game.
\end{proofatend}


\subsection{Alternative Form}

We are going to use an alternative form of this axiom in the fragment of the logic, more amenable to automated deduction techniques. The alternative axiom we will consider differ from the original axiom in two ways, that we describe below.

\subsubsection{Encryption Oracle Calls}
\todo{Why this form: for lemma $\beta_{i,l} \equiv \rtilde \beta_{i,l}[\beta_{j,l}]$ with $\forall o, \beta_{j,l}^o \not \in \condst(\rtilde \beta_{i,l}[]\downarrow_R)$} Instead of allowing any decryptions using keys in $\keys$ to appear in encryption oracle calls, we will require these decryptions to be guarded, to make sure that the decryptions are not performed on terms previously sent to the decryption oracle. Of course the resulting axiom is a specialization of the previous one, and is therefore valid. But it turns out that this is not a restriction in the following sense: for any decryption, there exists a semantically equal term that only uses guarded decryptions. We formalize this below.

\begin{definition} 
  For any finite set of key pairs $\keys$, we let $R_{\CCA_b}^\keys$ be the binary relation having the same definition than $R_{\CCA_a}^\keys$, apart for the encryption case that we replace by:
  \begin{enumerate}
    \setcounter{enumi}{1}
  \item \textbf{Encryption Case:} $x$ a fresh variable that does not appear in $\encvar \cup \decvar$, $\sk \in \keys$ and $\pk$ the corresponding public key:
    \begin{multline*}
      \left((\phi,\{u\}_{\pk}^{\nonce_r}),\encvar \cup \{x\},\decvar,\randmap \cup \{x \mapsto \nonce_r\}, \encmap \cup \{x \mapsto \{u\}_{\pk}^{\nonce_r}\} ,\decmap\right) \\
      R_{\CCA_b}^\keys  \left((\psi,\{v\}_{\pk}^{\nonce_r'}),\encvar \cup \{x\},\decvar,\randmap' \cup \{x \mapsto \nonce_r'\}, \encmap' \cup \{x \mapsto \{v\}_{\pk}^{\nonce'_{r}}\} ,\decmap'\right)
    \end{multline*}
    if there exist $t,t' \in \mathcal{T}(\sig, \mathcal{\encvar}')$ such that the following conditions hold:
    \begin{itemize}
    \item $(\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_b}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$
    \item $u \equiv t\decmap, \,v \equiv t'\decmap'$
    \item $\nodec(\keys;t,t')$ (this ensure that the only decryptions are calls to the oracle).
    \item $\fresh{\nonce_r,\nonce_r'}{\phi,u,\psi,v}$ and $\hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$
    \end{itemize}
  \end{enumerate}
\end{definition}

We first show the soundness of $\CCA_{b}$.
\begin{proposition}
  All formulas in CCA$_b$ are computationally valid if the encryption scheme is $\textsc{ind-cca}_2$ secure.
\end{proposition}

\begin{proof}
  We show that all instances of $CCA_{b}$ are instances of $CCA_{a}$ by induction on the definition of $R_{\CCA_b}^\keys$. As $R_{\CCA_b}^\keys$ and $R_{\CCA_a}^\keys$ coincide on case $1$ and $3$, we only need to check that when the conditions of the encryption case of $CCA_{b}$ hold, the conditions of the encryption case of $CCA_{a}$ hold.

  Using the notation of the definition, one can check that $u \equiv t\decmap, \,v \equiv t'\decmap'$ and $\nodec(\keys;t,t')$ implies that  $\keys \decpos u,v$. The result follows immediately.
\end{proof}

\begin{definition}
  Let $=_{\llbracket \rrbracket}$ be the relation defined on terms as follows: for all terms $t,t'$, we have $t =_{\llbracket \rrbracket} t'$ iff for every computational model $\cmodel$, $\llbracket t \rrbracket_{\cmodel} = \llbracket t' \rrbracket_{\cmodel}$.
\end{definition}

\begin{definition}
  Let $=_{eR}$ be the reflexive, symmetric and transitive closure of:
  \[
    =_R \cup 
    \left\{ 
      (t[\ite{\eq{u}{v}}{s[u]}{s'}],t[\ite{\eq{u}{v}}{s[v]}{s'}])
    \right\}
  \]
\end{definition}

\begin{proposition}
  $=_{eR}$ is valid: $=_{eR} \,\subseteq\, =_{\llbracket \rrbracket}$.
\end{proposition}

\begin{proof}
  This easily follows from the fact that:
  \[
    =_R \;\subseteq =_{\llbracket \rrbracket}
    \quad \text{ and }\quad
    \left\{ 
      (t[\ite{\eq{u}{v}}{s[u]}{s'}],t[\ite{\eq{u}{v}}{s[v]}{s'}])
    \right\} \;\subseteq\;=_{\llbracket \rrbracket}
  \]
  and that $=_{\llbracket \rrbracket}$ is a equivalence relation.
\end{proof}

We show the completeness of $R_{\CCA_b}^\keys$ with regards to the semantics, by showing that every instance of $R_{\CCA_a}^\keys$ is equal, modulo $=_{eR}$, to an instance of $R_{\CCA_b}^\keys$.
\begin{proposition}
  For all instance of $R_{\CCA_a}^\keys$:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  there exists $\rtilde \phi,\rtilde \psi,\rtilde \encmap,\rtilde \decmap,\rtilde \encmap',\rtilde \decmap'$ such that:
  \begin{itemize}
  \item $\rtilde \phi =_{eR} \phi$ and $\rtilde \psi =_{eR} \psi$.
  \item $\forall x \in \encvar, x\rtilde \encmap =_{eR} x \encmap$ (same for $\encmap'$) and $\forall x \in \decvar, x\rtilde \decmap =_{eR} x \decmap$ (same for $\decmap'$).
  \item This is an instance of  $R_{\CCA_b}^\keys$:
    \[
      (\rtilde \phi,\encvar,\decvar,\randmap,\rtilde \encmap,\rtilde \decmap) R_{\CCA_b}^\keys (\rtilde \psi,\encvar,\decvar,\randmap',\rtilde \encmap',\rtilde \decmap')
    \]
  \end{itemize}
\end{proposition}

\begin{proofatend}
  First observe that if we have:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_b}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  then we can assume w.l.o.g that all decryptions appearing in $\phi$ have been queried to the decryption oracle. Formally, for all $u \in \phi$, if there exists $s$ such that $\dec(s,\sk) \in \st(u)$ (with $\sk \in \keys$) then there exists $x \in \decvar$ such that $x\decmap \equiv \elses(l,\dec(s,\sk))$ where $l \equiv \eq{u}{x_1\rtilde \encmap},\dots,\eq{u}{x_n\rtilde \encmap}$ and $\{x_1,\dots,x_n\}$ is the subset of variables of $\encvar$ such that $x\rtilde \encmap$ is an encryption using public-key $\pk$. We make the same assumption on $\psi$.

  We now prove the proposition by induction on the definition of $R_{\CCA_a}^\keys$. The only interesting case is the second case, where the definitions of $R_{\CCA_a}^\keys$ and $R_{\CCA_b}^\keys$ differ: let $u,v$ be such that:\\[0.2em]
  \(
  \begin{array}{ll}
    \bullet & (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')\\
    \bullet & \keys \decpos u,v\\
    \bullet & \fresh{\nonce_r,\nonce_r'}{\phi,u,\psi,v}\\
    \bullet & \hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)\\
  \end{array}
  \)\\
  Let $\rtilde \phi,\rtilde \psi,\rtilde \encmap,\rtilde \decmap,\rtilde \encmap',\rtilde \decmap'$ obtained using the induction hypothesis on:
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  We are looking for terms $t,t'$ such that $t\rtilde \decmap =_{eR} u$ and $t'\rtilde \decmap' =_{eR} v$. 

  Let $x \in \decvar$, we know that $x\rtilde \decmap \equiv \elses(l,\dec(s,\sk))$ where $l \equiv \eq{u}{x_1\rtilde \encmap},\dots,\eq{u}{x_n\rtilde \encmap}$ and $\{x_1,\dots,x_n\}$ is the subset of variables of $\encvar$ such that $x\rtilde \encmap$ is an encryption using public-key $\pk$. Observe that we have:
  \[
    \dec(s,\sk) =_{eR} 
    \begin{alignedat}[t]{2}
      &\ite{\eq{u}{x_1\rtilde \encmap}}{x_1\rtilde\encmap\\ &}
      {
        \begin{alignedat}[t]{2}
          &\ite{\eq{u}{x_2\rtilde \encmap}}{x_2\rtilde\encmap\\ &
            \begin{alignedat}[t]{2}
              &\dots\\ &
            }{\begin{alignedat}[t]{2}
                &\ite{\eq{u}{x_n\rtilde \encmap}}{x_n\rtilde\encmap\\ &}
                {
                  (\elses(l,\dec(s,\sk)))
                }
              \end{alignedat}
            \end{alignedat}
          }
        \end{alignedat}
      }
    \end{alignedat}
  \]
  Let $v_x$ be the term in the right-hand side of the equality above, we have $v_x \equiv w_x[\elses(l,\dec(s,\sk))]$ where $w_x$ doe not contain $\dec(s,\sk)$ as a subterm. We then let $t$ be the term obtained from $u$ by replacing all decryption $\dec(s,\sk)$ (with $\sk \in \keys$) appearing in $u$ by $v_x$, where $x$ is such that $x\decmap \equiv \elses(\_,\dec(s,\sk))$ (recall that we assumed w.l.o.g that such an $x$ exists at the beginning of the proof).

  Hence $t\decmap =_{eR} u$ and $\nodec(\keys;t)$. Using the induction hypothesis we know that $\forall x \in \decvar, x\rtilde \decmap =_{eR} x \decmap$ therefore $t\rtilde \decmap =_{eR} u$. Similarly we can build a term $t'$ such that $t'\rtilde \decmap =_{eR} v$ and $\nodec(\keys;t')$. To conclude it only remains to show that the other syntactic side-conditions hold, which is straightforward since we did not touch to the nonces in $\encvar\randmap$ and $\encvar\randmap'$.
\end{proofatend}

\subsubsection{\texorpdfstring{$\CCA_c$}{CCAc}}

When adding a decryption call to a $R_{\CCA_b}^\keys$ instance, we add one guard $\eq{u}{x\encmap}$ for all $x \in \encvar$ such that $x\encmap$ is an encryption using public-key $\pk$, even though this encryption $x\encmap$ may not appear in $u$. 

For example, if $\encvar = \{x_0,x_1\}$ and $\encmap = \{x_0 \mapsto \alpha_0, x_1 \mapsto \alpha_1\}$ where $\alpha_i \equiv \enc{m_i}{\pk}{\nonce_i}$, then to guard $\dec(g(\alpha_1),\sk)$ we need to add two guards, $\eq{g(\alpha_0)}{m_0}$ and $\eq{g(\alpha_1)}{m_1}$. This yields the term:
\begin{alignat*}{2}
  \ite{&&\eq{g(\alpha_0)}{\alpha_0}}{&\zero(\dec(g(\alpha_1),\sk))\\
  }{\ite{&&\eq{g(\alpha_1)}{\alpha_1}}{&\zero(\dec(g(\alpha_1),\sk))\\
      &&}{&\dec(g(\alpha_1),\sk)}}
\end{alignat*}
But here, the adversary, represented by the adversarial function $g$, is computing the query to the decryption oracle using only one of the two previous calls to the encryption oracle, namely $\alpha_1$. Therefore there is no need to add the guard $\eq{g(\alpha_0)}{m_0}$, since $g$ has a negligible probability of returning $\alpha_0$. To remove unnecessary guards when building the decryption oracle call $\dec(u,sk)$, we require that $\eq{u}{\alpha}$ is added to the list of guards if and only if $\alpha \equiv \enc{\_}{\pk}{\nonce}$ ``appears'' in $u$, or more precisely the $R$-normal form of $u$ (to have a condition stable by $R$ rewritings). Formally, we do this by requiring that $\nonce \in \st(u\downarrow_R)$. For example, in this version of the $\CCA$ axiom the term $\dec(g(\alpha_1),\sk)$ is guarded by:
\begin{alignat*}{2}
  \ite{&&\eq{g(\alpha_1)}{\alpha_1}}{&\zero(\dec(g(\alpha_1),\sk))\\
    &&}{&\dec(g(\alpha_1),\sk)}
\end{alignat*}

Finally we add the following restriction: in the decryption case, when building the terms guarding $\dec(u,\sk)$ and $\dec(u',\sk)$, we require that there exists some term $t$ such that $u \equiv t\encmap\decmap$ and $v \equiv t\encmap'\decmap'$, and such that $t$ \emph{is if-free}. This is a restriction of the axiom, akin to the one we did for $\cs$. We can somehow quantify what we lose when doing the this: if we consider the logic with the \emph{generalized} $\cs$ axiom, then the version of the $\CCA$ axiom without the restriction that $t$ is if-free is admissible from the generalized $\cs$, $R$ and the restricted $\CCA$ axiom.

\begin{definition} 
  For any finite set of key pairs $\keys$, we let $R_{\CCA_c}^\keys$ be the binary relation having the same definition than $R_{\CCA_b}^\keys$, apart for the decryption case that we replace by:
  \begin{enumerate}
    \setcounter{enumi}{2}
  \item \textbf{Decryption Case:} Let $\sk \in \keys$, $\pk$ the corresponding public key and $z$ be a fresh variable:
    \begin{multline*}
      \left(\left(\phi,\elses(l,\dec(u,\sk))\right),\encvar,\decvar \cup \{z\},\randmap, \encmap,\decmap\cup \{z \mapsto \elses(l,\dec(u,\sk))\}  \right) \\
      R_{\CCA_a}^\keys  \left(\left(\psi,\elses(l',\dec(v,\sk))\right),\encvar,\decvar \cup \{z\},\randmap', \encmap',\decmap'\cup \{z \mapsto \elses(l',\dec(v,\sk))\}\right)
    \end{multline*}
    if there exists $t \in \mathcal{T}(\sig,\encvar \cup \decvar)$ such that the following conditions hold:
    \begin{itemize}
    \item $(\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_a}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')$
    \item $ u \equiv t\encmap\decmap$ and $v \equiv t\encmap'\decmap'$ and $t$ is if-free.
    \item $l \equiv \left(\eq{u}{y_1\encmap},\dots,\eq{u}{y_n\encmap}\right)$ where $\{y_1,\dots,y_m\} = \{x \in \encvar \mid x\encmap \equiv \enc{\_}{\pk}{\nonce_x} \wedge \nonce_x \in st(u\downarrow_R)\}$.
    \item $l' \equiv \left(\eq{v}{y'_1\encmap'},\dots,\eq{v}{y'_{n}\encmap'}\right)$ where $\{y'_1,\dots,y'_n\} = \{x \in \encvar \mid x\encmap' \equiv \enc{\_}{\pk}{\nonce_x} \wedge \nonce_x \in st(u'\downarrow_R)\}$.
    \item $\nodec(\keys;t) \text{ and } \hiddenr(\encvar\randmap \cup \encvar\randmap';\phi,u,\psi,v)$
    \end{itemize}
  \end{enumerate}
\end{definition}

Let $R_{\CCA_c'}^\keys$ defined as $R_{\CCA_c}^\keys$, but \emph{without} the restriction that $t$ is if-free. We show the completeness of $R_{\CCA_c'}^\keys$ with regards to the semantics, by showing that every instance of $R_{\CCA_b}^\keys$ is equal, modulo $=_{eR}$, to an instance of $R_{\CCA_c'}^\keys$.
\begin{proposition}
  For all instance of $R_{\CCA_b}^\keys$ such that all decryption are on 
  \[
    (\phi,\encvar,\decvar,\randmap,\encmap,\decmap) R_{\CCA_b}^\keys (\psi,\encvar,\decvar,\randmap',\encmap',\decmap')
  \]
  there exists $\rtilde \phi,\rtilde \psi,\rtilde \encmap,\rtilde \decmap,\rtilde \encmap',\rtilde \decmap'$ such that:
  \begin{itemize}
  \item $\rtilde \phi =_{eR} \phi$ and $\rtilde \psi =_{eR} \psi$.
  \item $\forall x \in \encvar, x\rtilde \encmap =_{eR} x \encmap$ (same for $\encmap'$) and $\forall x \in \decvar, x\rtilde \decmap =_{eR} x \decmap$ (same for $\decmap'$).
  \item This is an instance of  $R_{\CCA_c}^\keys$:
    \[
      (\rtilde \phi,\encvar,\decvar,\randmap,\rtilde \encmap,\rtilde \decmap) R_{\CCA_c'}^\keys (\rtilde \psi,\encvar,\decvar,\randmap',\rtilde \encmap',\rtilde \decmap')
    \]
  \end{itemize}
\end{proposition}

\begin{proof}
  \toadd{justification : $s[\cdots] =_R s[\cdots]\downarrow_R =_R s[\cdots]\{\nonce_r \mapsto 0\}$, hence $\eq{s[\cdots]}{\enc{\_}{\_}{\nonce_r}} =_{sem} \false$}
\end{proof}

We then show the soundness of CCA$_{c'}$, and as a corollary of CCA$_{c}$ which is included in CCA$_{c'}$.
\begin{proposition}
  All formulas in CCA$_{c'}$ are computationally valid if the encryption scheme is $\textsc{ind-cca}_2$ secure.
\end{proposition}

\begin{proof}
  \toadd{TODO}
\end{proof}

\begin{proposition}
  For all instance $\vec u \sim \vec u'$ of CCA$_{c'}$, there exists a proof of $\vec u \sim \vec u'$ using rules $R + CS_{\textsf{gen}} + \text{CCA}_{c}$, where $CS_{\textsf{gen}}$ is the unrestricted version of $CS$.
\end{proposition}

\begin{proof}
  \toadd{TODO}
\end{proof}

\begin{proposition}
  \label{prop:enc-differ} 
  \todo{Update to fit uses}
  Let $s^o$ and $s^1$ be two term, and assume that they are well-guarded in, respectively, $t^0 \equiv C^0[\vec g^0 \diamond (s^0_a)_a]$ and $t^1 \equiv C^1[\vec g^1 \diamond (s^1_a)_a]$ under $\ek$. Moreover assume that there exists $l_0,l_1$ such that $s^0_{l_0} \equiv s^1_{l_1}$. Then $t^0 \equiv t^1$.
\end{proposition}


\begin{proof}
  Let $\phi_\keys$ be the $\encs$-quasi substitution that replaces all occurrences of $\zero(\dec(u,\sk))$ by $\dec(u,\sk)$ if $\sk \in \keys$. Let $s^0_p$ be the right-most element of $t^0$, and $s^1_q$ be the right-most element of $t^1$. Observe that since $s^0$ is well-guarded in $t^0$ under $\ek$ we have $\phi_\keys(s^0_{l_0}) \equiv s^0_p$, and similarly $\phi_\keys(s^1_{l_1}) \equiv s^1_q$. Therefore $s^0_p \equiv s^1_q$. Since for every term $s$ there exists a unique term $t$ such that $s$ is well-guarded in $t$ under $\ek$, we know that $t^0 \equiv t^1$.
\end{proof}


\begin{proposition}
  \label{prop:cca-length}
  For all $b,b' \in \mathcal{T}(\sig)$, if $\vec w,\enc{\ite{b}{u}{v}}{pk}{r} \sim \vec w',\enc{t'}{pk'}{r'}$ is a valid application of the \cca axiom where the right-most element is a LR oracle call, and if $b$ is not a guard
  then $\vec w,\enc{u}{pk}{r} \sim \vec w',\enc{t'}{pk'}{r'}$ and $\vec w,\enc{v}{pk}{r} \sim \vec w',\enc{t'}{pk'}{r'}$ are valid applications of the \cca axiom.
\end{proposition}

\begin{proof}
  Since this is a valid application of the \cca axiom we know that $\eql{\ite{b}{u}{v}}{t'}$ is derivable. Therefore using the branch invariance property we know that:
  \[
    \eql{u}{t'} \text{ and }\eql{v}{t'}
  \]
  are derivable. This shows that the length constraints holds. As all the other constraints are subterm, therefore we know that  $\vec w,\enc{u}{pk}{r} \sim \vec w',\enc{t'}{pk'}{r'}$ and $\vec w,\enc{v}{pk}{r} \sim \vec w',\enc{t'}{pk'}{r'}$ are valid applications of the \cca axiom.
\end{proof}

\paragraph{Axiom of the logic}
We let $\CCA$ be the closure of $\CCA_c$ under $\restr$. An interesting property is that any instance $\vec u \sim \vec v$ of $\CCA$ can be extended into an instance $\vec u' \sim \vec v'$ of $\CCA_c$, with at most a polynomial increase in size.

\begin{proposition}
  \label{prop:cca-small-restr}
  For all instance $\vec u \sim \vec v$ of $\CCA$, there exists $\vec u_1,\vec v_1$ such that $\vec u,\vec u_1 \sim \vec v,\vec v_1$ is an instance of $\CCA_c$ (modulo $\perm$) and $|\vec u_1| + |\vec v_1|$ is of polynomial size in $|\vec u| + |\vec v|$.
\end{proposition}

\begin{proof}
  Let $\vec u \sim \vec v$ be an instance of $\CCA$, and $\vec w,\vec w'$ be such that $\vec u,\vec w \sim \vec v,\vec w'$ is the corresponding instance of $\CCA_c$ (modulo $\perm$). Our goal is to find $\vec u_1 \subseteq \vec w$ and $\vec v_1 \subseteq \vec w'$ such that $\vec u,\vec u_1 \sim \vec v,\vec v_1$ is an instance of $\CCA_c$ (modulo $\perm$) and $|\vec u_1| + |\vec v_1|$ is of polynomial size in $|\vec u| + |\vec v|$.
  
  When we applied the restriction axioms we may have removed encryptions or decryptions in $\vec w \sim \vec w'$ that are used to build terms later one in $\vec u \sim \vec v$. We only need to add the terms $\vec u_1$ of $\vec w$ (resp. $\vec v_1$ of $\vec w'$) that are subterms of $\vec u$ (resp. $\vec v$). This ensures that we have an instance of $\CCA_c$ and that we add, in the worst case, a linear number of terms (therefore $|\vec u_1| + |\vec v_1|$ is of quadratic size in $|\vec u| + |\vec v|$).
\end{proof}

\subsection{Proof Example}
\input{examples}

\FloatBarrier

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ms"
%%% End:


==> proofatend.tex <==
% Original author: egreg
% Source: https://tex.stackexchange.com/a/33230
% Modified by: Adrien Koutsos

\usepackage{etex,etoolbox}
\usepackage{amsthm,amssymb}
\usepackage{thmtools}
\usepackage{environ}
\usepackage{hyperref}

\makeatletter
% \providecommand{\@fourthoffour}[4]{#4} % Standard version
\providecommand{\@fourthoffour}[3]{#3} % ACM SIGPLAN version
% We define an addition for the theorem-like environments; when
% \newtheorem{thm}{Theorem} is declared, the macro \thm expands
% to {...}{...}{...}{Theorem} and with \@fourthoffour we access
% to it; then we make available \@currentlabel (the theorem number)
% also outside the environment.  
\newcounter{counttheorems}

\theoremstyle{definition}
\newtheorem{myproof}{Proof}


\newcommand\fixstatement[2][\proofname\space of]{%
  \ifcsname thmt@original@#2\endcsname
    % the theorem has been declared with \declaretheorem
    \AtEndEnvironment{#2}{%
      \xdef\pat@uniqlabel{\thecounttheorems}%
      \xdef\pat@label{\expandafter\expandafter\expandafter
        \@fourthoffour\csname thmt@original@#2\endcsname\space\@currentlabel}%
      \xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
      \addtocounter{counttheorems}{1}
      \expandafter\label{thm_uniq:\pat@uniqlabel}
    }%
  \else
    % the theorem has been declared with \newtheorem
    \AtEndEnvironment{#2}{%
      \xdef\pat@uniqlabel{\thecounttheorems}%
      \xdef\pat@label{\expandafter\expandafter\expandafter
        \@fourthoffour\csname #1\endcsname\space\@currentlabel}%
      \xdef\pat@proofof{\@nameuse{pat@proofof@#2}}%
      \addtocounter{counttheorems}{1}
      \expandafter\label{thm_uniq:\pat@uniqlabel}
    }%
  \fi
  \@namedef{pat@proofof@#2}{#1}%
}

% We allocate a block of 1000 token registers; in this way \prooftoks
% is 1000 and we can access the following registers of the block by
% \prooftoks+n (0<n<1000); we'll use a dedicated counter for it
% that is stepped at every proof
\globtoksblk\prooftoks{1000}
\newcounter{proofcount}

% We gather the contents of the proof as argument to \proofatend
% and then we store
% "\begin{proof}[Proof of <theoremname> <theoremnumber>]#1\end{proof}"
% in the next token register of the allocated block
\NewEnviron{proofatend}
  {\proof See Proof~\ref{pr:\pat@uniqlabel}.\endproof
  \edef\next{\noexpand\begin{myproof}[Proof of \noexpand\autoref{thm_uniq:\pat@uniqlabel}]\noexpand\label{pr:\pat@uniqlabel}}%
  \toks@=\expandafter{\next}%
  \global\toks\numexpr\prooftoks+\value{proofcount}\relax=
  \expandafter{\the\expandafter\toks@\BODY%
  \qed\end{myproof}}%
  \stepcounter{proofcount}}

% We gather the contents of the proof as argument to \proofatend
% and then we store
% "\begin{proof}[Proof of <theoremname> <theoremnumber>]#1\end{proof}"
% in the next token register of the allocated block
\NewEnviron{proofatendsection}
  {\label{sec:\pat@uniqlabel}
  \edef\next{\noexpand\subsection{Proofs of Section~\noexpand\ref{sec:\pat@uniqlabel}}}%
  \toks@=\expandafter{\next}%
  \global\toks\numexpr\prooftoks+\value{proofcount}\relax=
  \expandafter{\the\expandafter\toks@\BODY%
  }%
  \stepcounter{proofcount}}



% \printproofs simply loops over the used token registers of the
% block, freeing their contents
\def\printproofs{%
  \count@=\z@
  \loop
    \the\toks\numexpr\prooftoks+\count@\relax
    \ifnum\count@<\value{proofcount}%
    \advance\count@\@ne
  \repeat}
\makeatother

% % Here starts the example, with two theorem declarations
% \declaretheorem[style=plain,name=Theorem,qed=$\square$,numberwithin=section]{thm}
% %\declaretheorem[style=plain,name=Lemma,qed=$\square$,numberlike=thm]{lem}
% %\newtheorem{thm}{Theorem}
% \newtheorem{lem}[thm]{Lemma}
% \fixstatement{thm}
% \fixstatement[Demonstration of]{lem}


% \begin{document}
% \begin{lem}\label{addition}
% $1+1=2$
% \end{lem}
% \begin{proofatend}
% It's quite clear.
% \end{proofatend}

% \begin{thm}
% $1+2=3$
% \end{thm}
% \begin{proofatend}
% Obvious from lemma \ref{addition}.
% \end{proofatend}

% \section*{Proofs}

% \printproofs


==> undecidability-fafrag.tex <==
We let \fafrag be the restriction of our logic to the rules $FA$, $Duplicate, Sym$ and $Subst$, the unitary axioms $Refl \cup Ind_{CCA2}$ modulo the term rewriting system $R$.

Having a proof of $u \sim v$ using only the $FA$ rule (plus $Duplicate, Sym$ and $Subst$), unitary axioms $UA$ and modulo the term rewriting system $T$ can be re-formulated as follows: is there an unitary axiom $\vec u \sim \vec v$ in $UA$ and a many-holed context $C$ such that $u \leftrightarrow_T^* C[\vec u]$ and $v \leftrightarrow_T^* C[\vec v]$ (this reformulation stems from the fact that rewritings can always be pushed to the conclusion of the derivation).

This problem turns out to be undecidable, even if there is only one unitary axiom, by reduction from the Post Correspondence Problem.
\begin{theorem}\label{thm:und}
The following problem is undecidable:\\
\textbf{Input:} A convergent term rewriting system $\ra$, a list of pairs of closed terms $(u_i,v_i)_{1 \le i \le n}$ and two closed terms $u,v$.\\
\textbf{Question:} There exists a context $C$ with $n$ holes such that $C[u_1,\dots,u_n] \leftrightarrow^* u$ and $C[v_1,\dots,v_n] \leftrightarrow^* v$.
\end{theorem}

\begin{proof}
See Fig.~\ref{fig:undproof}.
\end{proof}

\begin{figure}[htp]
\begin{center}
\includegraphics[width=0.5\linewidth]{undecidable}
\end{center}
\caption{\label{fig:undproof} Undecidability proof of Theorem~\ref{thm:und}}
\end{figure}

\FloatBarrier

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ms"
%%% End:


